Time Warp: The Gap Between Developers' Ideal vs Actual Workweeks in an AI-Driven Era

Software developers balance a variety of different tasks in a workweek, yet the allocation of time often differs from what they consider ideal. Identifying and addressing these deviations is crucial for organizations aiming to enhance the productivity and well-being of the developers. In this paper, we present the findings from a survey of 484 software developers at Microsoft, which aims to identify the key differences between how developers would like to allocate their time during an ideal workweek versus their actual workweek. Our analysis reveals significant deviations between a developer's ideal workweek and their actual workweek, with a clear correlation: as the gap between these two workweeks widens, we observe a decline in both productivity and satisfaction. By examining these deviations in specific activities, we assess their direct impact on the developers' satisfaction and productivity. Additionally, given the growing adoption of AI tools in software engineering, both in the industry and academia, we identify specific tasks and areas that could be strong candidates for automation. In this paper, we make three key contributions: 1) We quantify the impact of workweek deviations on developer productivity and satisfaction 2) We identify individual tasks that disproportionately affect satisfaction and productivity 3) We provide actual data-driven insights to guide future AI automation efforts in software engineering, aligning them with the developers' requirements and ideal workflows for maximizing their productivity and satisfaction.

==> Sections/Abstract.tex <==
Software developers balance a variety of tasks in a workweek, yet the allocation of time often differs from what they consider ideal. Identifying and addressing these deviations is crucial for organizations aiming to enhance both productivity and employee well-being.
In this paper we present the findings from a survey that aims to identify the key differences between how software engineers allocate their time during an ideal workweek versus their actual workweek. Our analysis reveals significant deviations between a developers' ideal workweek and their actual workweek, with a clear correlation: as the gap between these two workweeks widens, we observe a decline in in both productivity and satisfaction. By examining these deviations in specific activities, we assess their direct impact on the developers' satisfaction and productivity. Additionally, given the growing adoption of AI tools in software engineering, both in the industry and academia, we identify specific tasks and areas that could be strong candidates for automation. 
Our work makes three key contributions: 1) We quantify the impact of workweek deviations on developer productivity and satisfaction 2) We identify individual tasks that disproportionately affect satisfaction and productivity. 3) We provide actual data-driven insights to guide future AI automation efforts in software engineering, aligning them with the developers' requirements and ideal workflows to maximize productivity, satisfaction and impact.  

==> Sections/Introduction.tex <==
In this paper, we a present the findings from our study aimed at analyzing the differences between a developers' `ideal' and `actual' workweek.
Our study confirms and builds upon previous research in this area, that explore developers' typical and good workdays \cite{8666786}. By observing these deviations at a workweek level, we manage to capture the cumulative effect of task-allocation, while giving a fine-grained view by exploring the activity level influences. 
To the best of our knowledge, our study is the first work that focuses on how deviations, both at the overall workweek and individual activity levels, affect developers' productivity and satisfaction. Our research additionally quantifies how deviations across different activities impact self-reported developer productivity and satisfaction. We also explore how AI tool usage influences the productivity and satisfaction of developers. In addition to that, we systematically analyze and present the developers' feedback on which tasks they would prefer to see automated using AI, providing valuable insights for future AI tool development. 

==> Sections/Methodology.tex <==
\section{Methodology}
In this section, we outline the key research questions driving this study, followed by a detailed description of the methodology used to design and conduct the survey.
\subsection{Research Questions}
\begin{enumerate}
    \item[\textbf{RQ1:}] How do developers allocate their time during a typical workweek, and how does this compare to their perception of an \textbf{ideal workweek?}
    \item[\textbf{RQ2:}] How are developer's satisfaction and productivity affected by \textbf{deviations} from their ideal workweek?
     \item[\textbf{RQ3:}] For which tasks do developers prefer using \textbf{AI tools}, and how does the frequency of AI tool usage \textbf{influence} their satisfaction and productivity?
\end{enumerate}

\subsection{Survey Design}
% Describe how the survey was conducted, survey structure, sample size, which activities were selected and how, incentives, etc. 

To gain insights into the types of activities developers engage in during a typical work week, we conducted a series of exploratory interviews with 12 randomly selected participants. These semi-structured interviews provided a qualitative foundation, allowing us to iteratively develop a comprehensive list of higher-level activities that reflect both ideal and actual workweek allocations. The findings from these interviews were instrumental in refining our survey questions and design.

% - When was it distributed
% - How many people were invited
% - how was the survey advertised
% - incentive provided to participants
% - how many responses received (with response rates)
% - Board of ethics description \& instruments
% - Describe the main questions asked in the survey

The survey was distributed in \textcolor{blue}{May 2024} to software engineers working in Microsoft teams across India and the United States. A total of 6000 developers were invited to participate via email. Framed as a study aimed at boosting developer productivity by understanding how they allocate their time in a workday, the survey received 510 complete responses (responses rate of 8.5\%). After finishing the survey, the participants could enter a sweepstake to win one out of ten \$50 Amazon.com Gift Cards.
\textcolor{blue}{description of ethics}.

The main questions in the survey were as follows:
\begin{enumerate}
    \item Their roles and years of experience in the industry/team
    \item The hours spent on various activities in their typical workweek
    \item Ideally, the percentage of time they would want to allocate to each activity in a workweek
    \item How productive and satisfied were they by their past workweek
    \item Activities they find most cognitively challenging
    \item How often do they use AI tools to assist in their daily activities
    \item Two open-ended questions about the activities they would want to automate using AI tools, and advice for new hires to boost their productivity and satisfaction levels 
\end{enumerate}



\subsection{Data Analysis \& Exploration}
% Here, we could start with discussing the survey group:
% - demographic observations
% - distribution of participants (based on the years experience in the industry/team), 

From the exploratory interviews, we identified sixteen key activities, which were subsequently used to quantify the developers' time allocation across their work week. 

\subsection{Limitations}

==> Sections/RQ3.tex <==
\subsection{Which tasks do developers want to automate?}

In the survey, we asked the developers to answer the question \textit{``Which of your current tasks would you most like to see automated? Which processes do you think could be enhanced to minimize repetitive work?"} 

We received 242 open-ended responses from the developers. To analyze the responses, we utilized the GPT-4 model to identify an initial set of task categories highlighted in the data. The model identified 17 distinct categories. To ensure comprehensive coverage, we uniformly sampled 60 responses based on their length. Four annotators independently reviewed these responses using a closed-coding approach. 
They assigned labels to each response based on the initial categories suggested by GPT-4, while also identifying any new categories that emerged during the process. 
The inter-rater agreement, measured using the Jaccard similarity metric, was 81.5\%, indicating a substantial level of agreement among annotators. Additionally, through discussions, the annotators agreed to introduce one new category (``Cloud Infrastructure Maintenance''), resulting in a list of 18 categories of tasks that developers would like to automate using AI. 
The remaining 182 responses were distributed equally amongst the four annotators and manually labelled using the extended taxonomy to identify the frequency of each category.

The final categories are summarized in \cref{tab:AutomationTasks}. For each category, we provide the name and a short description.
The table also illustrates the results from the manual annotation process and the frequency of each category. 
Documentation emerged as the most frequent category in our analysis of tasks that could be automated with AI. Developers suggested the use of AI to create and update documentation, maintain team knowledge bases, and also to efficiently understand existing code and systems from the available information. For example, D302 highlighted the importance of efficient documentation by saying: \textit{``I would love to see automated documentation of infrastructure and code. A lot of time is lost trying to understand the current resources that go into securing, building, and deploying our products and trying to understand how the different parts of our code base interact and depend on each other. It'd really lessen the cognitive load if this was well-documented in a way that is automatically kept up-to-date."} Similarly, developer D165 expresses the growing need for automating code documentation to keep pace with the rapid development cycles: \textit{``I would love it if there were some way to automatically generate architectural documentation or either a data flow or call stack diagram based on the structure of the actual code in the repository. While tools like CodeFlow exist for VSCode and Visual Studio, there's a learning curve and the lack of reward for better internal documentation means creating and updating documentation is on a volunteer basis. This, and the rapid pace of development means that onboarding any new engineer or existing engineer to a new area is a time-consuming manual process of last-minute documentation updates, or passing down tribal knowledge verbally. Would be nice if there were some way to tie internal documentation to a particular code base, so that every PR also `refreshes' the internal documentation or diagrams."} 

Following this, several developers emphasized the need for automating tasks associated with the setup and maintenance of development environments, which often involve complex processes such as configuring SSH keys, installing software dependencies, and initializing new development instances. Developer D81 points out the current challenges, stating, \textit{``Setting up the Dev. environment could be way simpler. Right now it is somewhat involved, time consuming, and brittle."} 
Similarly, Developer D403 emphasizes the significant impact of automation on productivity, noting, \textit{``Setting up a development environment takes up a huge amount of time in the development cycle, hence I feel that enhancing the same will greatly boost developer productivity"}


 Following closely are tasks related to  `Write/maintain tests', `Task Tracking \& Backlog Management', `Security \& Compliance', `Incident/Customer Issue Management', and `Communication'. This suggests that developers would like to use AI for tasks that support their core work of writing code.

Following are a few selected responses from developers discussing the activities which they want to see automated using AI. Developer D327 provides an elaborate description of the tasks to automate: \textit{`` b) A lot of my time goes into setting up Dev. environment to start working on a new PR or update old PR and merging the changes and building takes a lot of time (sometimes 2 hours) which hinders my productivity and sometimes is the reason why I procrastinate. c) We have weekly OCE (On-Call Engineering) rotations in our team where we have to create reports of the incidents we receive. I want the report generation to be automated. It’ll be such a big boost in our productivity."}.


==> Sections/table_backup.tex <==
\begin{table}
\centering
\caption{OLS Regression Results - Productivity \sukrit{Should we highlight stat sig findings ? }}
\begin{tabular}{lcccc}
\toprule
\textbf{Variable} & \textbf{coef} & \textbf{std err} & \textbf{t} & \textbf{P}\( > |t| \) \\
\midrule
\textbf{const}                          & 4.1078 & 0.055  & 74.621  & 0.000  \\
\textbf{diff\_Arch. \& Design}          & 0.0009 & 0.003  & 0.355   & 0.723  \\
\textcolor{darkgreen}{\textbf{diff\_Coding}}                   & \textcolor{darkgreen}{0.0061} & 0.002  & 3.027   & 0.003  \\
\textcolor{darkred}{\textbf{diff\_Dev. Environment}}         & \textcolor{darkred}{-0.0158} & 0.005  & -3.422  & 0.001  \\
\textcolor{darkgreen}{\textbf{diff\_Docs}}                     & \textcolor{darkgreen}{0.0103} & 0.005  & 1.995   & 0.047  \\
\textbf{diff\_PR/Code Review}           & -0.0046 & 0.006  & -0.803  & 0.423  \\
\textcolor{darkgreen}{\textbf{diff\_Refactoring}}              & \textcolor{darkgreen}{0.0130} & 0.004  & 2.935   & 0.003  \\
\textbf{diff\_Debugging}                & -0.0021 & 0.003  & -0.643  & 0.521  \\
\textbf{diff\_Monitoring \& Dashboards} & 0.0063 & 0.005  & 1.197   & 0.232  \\
\textbf{diff\_Testing}                  & 0.0045 & 0.004  & 1.093   & 0.275  \\
\textbf{diff\_Security \& Compliance}   & -0.0033 & 0.002  & -1.431  & 0.153  \\
\textbf{diff\_Customer Support}          & -0.0051 & 0.003  & -1.651  & 0.099  \\
\textcolor{darkred}{\textbf{diff\_Comm.}}                    & \textcolor{darkred}{-0.0079} & 0.004  & -2.120  & 0.034  \\
\textbf{diff\_Task Mgmt.}               & -0.0149 & 0.010  & -1.451  & 0.147  \\
\textbf{diff\_Tech-Talks}               & 0.0001 & 0.012  & 0.011   & 0.992  \\
\textbf{diff\_Mentoring/Onboarding}     & 0.0007 & 0.006  & 0.119   & 0.905  \\
\textcolor{darkgreen}{\textbf{diff\_Learning Tech.}}           & \textcolor{darkgreen}{0.0118} & 0.005  & 2.372   & 0.018  \\
\bottomrule
\label{tab:regression_results_productivity}
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{OLS Regression Results - Satisfaction}
\begin{tabular}{lcccc}
    \toprule
        & \textbf{coef} & \textbf{std err} & \textbf{t} & \textbf{P}\( > |t| \) \\
        \midrule
        \textbf{const} & 4.0436 & 0.061 & 66.061 & 0.000 \\
        \textbf{diff\_Arch. \& Design} & 0.0057 & 0.003 & 1.950 & 0.052 \\
        \textbf{diff\_Coding} & 0.0043 & 0.002 & 1.907 & 0.057 \\
        \textcolor{darkred}{\textbf{diff\_Dev. Environment}} & \textcolor{darkred}{-0.0151} & 0.005 & -2.935 & 0.004 \\
        \textcolor{darkgreen}{\textbf{diff\_Docs}} & \textcolor{darkgreen}{0.0161} & 0.006 & 2.803 & 0.005 \\
        \textcolor{darkred}{\textbf{diff\_PR/Code Review}} & \textcolor{darkred}{-0.0133} & 0.006 & -2.086 & 0.038 \\
        \textcolor{darkgreen}{\textbf{diff\_Refactoring}} & \textcolor{darkgreen}{0.0128} & 0.005 & 2.584 & 0.010 \\
        \textbf{diff\_Debugging} & -0.0010 & 0.004 & -0.267 & 0.789 \\
        \textbf{diff\_Monitoring \& Dashboards} & -0.0098 & 0.006 & -1.692 & 0.091 \\
        \textbf{diff\_Testing} & 0.0031 & 0.005 & 0.684 & 0.494 \\
        \textcolor{darkred}{\textbf{diff\_Security \& Compliance}} & \textcolor{darkred}{-0.0090} & 0.003 & -3.470 & 0.001 \\
        \textbf{diff\_Customer Support} & -0.0065 & 0.003 & -1.900 & 0.058 \\
        \textcolor{darkred}{\textbf{diff\_Comm.}} & \textcolor{darkred}{-0.0129} & 0.004 & -3.114 & 0.002 \\
        \textbf{diff\_Task Mgmt.} & 0.0085 & 0.011 & 0.743 & 0.458 \\
        \textbf{diff\_Tech-Talks} & -0.0032 & 0.013 & -0.243 & 0.808 \\
        \textbf{diff\_Mentoring/Onboarding} & 0.0077 & 0.007 & 1.142 & 0.254 \\
        \textcolor{darkgreen}{\textbf{diff\_Learning Tech.}} & \textcolor{darkgreen}{0.0126} & 0.006 & 2.279 & 0.023 \\
        \bottomrule
    \end{tabular}
    \label{tab:regression_results_satisfaction}
\end{table}
